Effect of tip speed ratio on multiscale coherent dynamics in the near wake of a model wind turbine

The near wake of a small-scale wind turbine is investigated using Particle Image Velocimetry (PIV) experiments at different tip speed ratios ($\lambda$). The wind turbine model had a nacelle and a tower mimicking real scale wind turbines. The near wake is found to be dominated by multiple coherent structures including the tip vortices, distinct vortex sheddings from the nacelle and tower, and wake meandering. The merging of the tip vortices is found to be strongly dependent on $\lambda$. A convective length scale ($L_c$) related to the pitch of the helical vortices is defined which is shown to be a better length scale than turbine diameter ($D$) to demarcate the near wake from the far wake. The tower induced strong vertical asymmetry in the flow by destabilising the tip vortices and promoting mixing in the lower (below the nacelle) plane. The nacelle's shedding is found to be important in 'seeding' wake meandering which although not potent, exists close to the nacelle, and it becomes important only after a certain distance downstream ($x>3L_c$). A link between the 'effective porosity' of the turbine and $\lambda$ is established and the strength and frequency of wake meandering is found to be dependent on $\lambda$. In fact, a decreasing trend of wake meandering frequency with $\lambda$ is observed, similar to vortex shedding from a porous disk at varying porosity. Such similarity upholds the notion of wake meandering being a global instability of the turbine, which can be considered as a 'porous' bluff body of diameter $D$.

==> README <==

  The ulem package provides various types of underlining that can stretch
  between words and be broken across lines in LaTeX or plain TeX.
  In LaTeX ulem replaces italics with underlining in \em-phasized text.
  A declaration of \normalem (or the \usepackage option "normalem") restores 
  the normal \em and \emph behavior.

  Copyright 1989-2019 by Donald Arseneau (Vancouver, Canada; asnd@triumf.ca)

  This software may be freely transmitted, reproduced, or modified for any
  purpose provided that this copyright notice is left intact.  

